AirCode: Unobtrusive Physical Tags for Digital Fabrication

We present AirCode, a technique that allows the user to tag physically fabricated objects with given information. An AirCode tag consists of a group of carefully designed air pockets placed beneath the object surface. These air pockets are easily produced during the fabrication process of the object, without any additional material or postprocessing. Meanwhile, the air pockets affect only the scattering light transport under the surface, and thus are hard to notice to our naked eyes. But, by using a computational imaging method, the tags become detectable. We present a tool that automates the design of air pockets for the user to encode information. AirCode system also allows the user to retrieve the information from captured images via a robust decoding algorithm. We demonstrate our tagging technique with applications for metadata embedding, robotic grasping, as well as conveying object affordances.

==> Makefile <==
# name of latex document
MAINDOC := uist

# latex source file
TEXSRC := uist.tex abstract.tex intro.tex overview.tex theory.tex \
          codes.tex imaging.tex related.tex application.tex results.tex \
	  app.tex conclusion.tex suppl.tex
BIBSRC := $(wildcard *.bib)

ifneq ($(strip $(BIBSRC)),)
BBLSRC := $(MAINDOC).bbl
endif

# latex program
TEX      := latex
PDFLATEX := pdflatex
BIB      := bibtex

# flags
TEX_FLAGS :=
PDF_FLAGS :=
BIB_FLAGS :=

#=====================================================#
# Display Codes (this is so we can track passes)
#=====================================================#
MOVE_TO_COL	= @echo  "\\033[60G"
SETCOLOR_RED 	= @echo  "\\033[0;31m"
SETCOLOR_GREEN 	= @echo  "\\033[0;32m"
SETCOLOR_BLUE	= @echo  "\\033[0;34m"
SETCOLOR_BACK	= @echo  "\\033[0m"

all: $(MAINDOC).pdf

pdf: $(MAINDOC).pdf

dvi: $(MAINDOC).dvi

full: $(BBLSRC) $(TEXSRC)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)
	$(SETCOLOR_GREEN)
	@echo "=========================FINAL PASS=============================="
	$(SETCOLOR_BACK)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)
	
	# require gs: ghostscript installed
	./compress.sh $(MAINDOC).pdf

	# pip2 install pypdf pdfsplit
	pdfsplit -o "./aircode_suppl.pdf" 12:14 $(MAINDOC).pdf
	pdfsplit -o "./aircode_main.pdf" 0:12 $(MAINDOC).pdf


%.dvi : %.aux
	$(SETCOLOR_BLUE)
	@echo "=========================AUX -> DVI PASS=============================="
	$(SETCOLOR_BACK)
	@$(TEX) $(TEX_FLAGS) $(*F)
	
$(MAINDOC).bbl : $(BIBSRC) $(TEXSRC) 
ifneq ($(strip $(BIBSRC)),)
	$(SETCOLOR_GREEN)
	@echo "=========================LaTeX PASS=============================="
	$(SETCOLOR_BACK)
	$(PDFLATEX) $(TEX_FLAGS) $(MAINDOC)
	$(SETCOLOR_GREEN)
	@echo "=========================BibTex PASS=============================="
	$(SETCOLOR_BACK)
	@$(BIB) $(BIB_FLAGS) $(MAINDOC)
endif

$(MAINDOC).pdf : $(TEXSRC)
	$(SETCOLOR_GREEN)
	@echo "=========================SINGLE PASS=============================="
	$(SETCOLOR_BACK)
	@$(PDFLATEX) $(PDF_FLAGS) $(MAINDOC)

.PHONY: all clean

clean:
	-$(RM) *.aux *.pdf *.bbl *.blg *.log


==> app.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=0.95\columnwidth]{figs/curve.pdf}
  \vspace{-1mm}
  \caption{ 
      {\bf (a)} The transmissive albedo of a scattering material (the 3D printing material we used) as a function of its thickness $d$.
      {\bf (b)} The contrast between a surface point above an air pocket with
      respect to a surface point without one, plotted as a function of the thickness $h$ of the air pocket.
      The three curves are plotted for different thickness $d$ of top material layer.
  \label{fig:tran_curve}}
  \vspace{-4mm}
\end{figure}


\section{Computing Transmission Profile $T_d(r)$}\label{app:trans}
We follow the Kubelka-Munk theory to compute the transmission profile $T_d(r)$
of a laterally infinite slab with a thickness $d$~\cite{cortat2004kubelka,HasanFMPR10}.
We measure the reflection and transmission profiles $R_D(r)$ and $T_D(r)$ of a slab with a thickness $D$,
and compute their Hankel transforms $\calR_D$ and $\calT_D$. Then, $\calR_d$ and $\calT_d$ of
an arbitrary thickness $d$ can be computed as
$$
\calR_d = \frac{S(d)}{\alpha S(d) + \beta C(d)}\;\text{ and }\; 
\calT_d = \frac{\beta}{\alpha S(d) + \beta C(d)},
$$
where $S(d)=\sinh(\gamma d)$ and $C=\cosh(\gamma d)$ are hyperbolic functions,
and 
$$
\alpha = 1 + \frac{\mathcal{K}}{\mathcal{C}},\;\;\beta=\sqrt{\alpha^2-1},\;\;\gamma=\sqrt{\mathcal{K}(\mathcal{K}+2\mathcal{S})}.
$$
Here both $\mathcal{S}$ and $\mathcal{K}$ are constant values, computed by
$$
\mathcal{S} = \lim_{d\to0}\frac{\mathcal{R}_d}{d}\;\;\text{ and }\;\;
\mathcal{K} = \lim_{d\to0}\frac{1-\mathcal{R}_d-\mathcal{T}_d}{d}.
$$
The limits here can be computed by repeatedly halving the thickness $d$ (starting from $\mathcal{R}_D$ and $\mathcal{T}_D$)
using the relationship~\eqref{eq:composite}. 

